Reducing Initial Cell-search Latency in mmWave Networks

Millimeter-wave (mmWave) networks rely on directional transmissions, in both control plane and data plane, to overcome severe path-loss. Nevertheless, the use of narrow beams complicates the initial cell-search procedure where we lack sufficient information for beamforming. In this paper, we investigate the feasibility of random beamforming for cell-search. We develop a stochastic geometry framework to analyze the performance in terms of failure probability and expected latency of cell-search. Meanwhile, we compare our results with the naive, but heavily used, exhaustive search scheme. Numerical results show that, for a given discovery failure probability, random beamforming can substantially reduce the latency of exhaustive search, especially in dense networks. Our work demonstrates that developing complex cell-discovery algorithms may be unnecessary in dense mmWave networks and thus shed new lights on mmWave system design.

==> Components/MetaFiles/acronyms.tex <==
%\chapter*{Acronyms}
%\renewcommand{\titulonome}{Acronyms}%
%\renewcommand{\prepbynome}{UFC.33 Team}%

%\begin{singlespace}
\begin{acronym}[LTE-Advanced]%\addtolength{\itemsep}{-0.5\baselineskip}
  \acro{2G}{Second Generation}
  \acro{3G}{3$^\text{rd}$~Generation}
  \acro{3GPP}{3$^\text{rd}$~Generation Partnership Project}
  \acro{4G}{4$^\text{th}$~Generation}
  \acro{5G}{5$^\text{th}$~Generation}
  \acro{AoA}{angle of arrival}
  \acro{AoD}{angle of departure}
  \acro{BER}{bit error rate}
  \acro{BF}{beamforming}
  \acro{BLER}{BLock Error Rate}
  \acro{BPC}{Binary Power Control}
  \acro{BPSK}{Binary Phase-Shift Keying}
  \acro{BRA}{Balanced Random Allocation}
  \acro{BS}{base station}
  \acro{CAP}{Combinatorial Allocation Problem}
  \acro{CAPEX}{Capital Expenditure}
  \acro{CBF}{Coordinated Beamforming}
  \acro{CS}{Coordinated Scheduling}
  \acro{CSI}{channel state information}
  \acro{CSIT}{channel state information at the transmitter}
  \acro{CSIR}{channel state information at the receiver}
  \acro{D2D}{device-to-device}
  \acro{DCA}{Dynamic Channel Allocation}
  \acro{DE}{Differential Evolution}
  \acro{DFT}{Discrete Fourier Transform}
  \acro{ULA}{uniform linear array}
  \acro{DIST}{Distance}
  \acro{DL}{downlink}
  \acro{DMA}{Double Moving Average}
  \acro{DMRS}{Demodulation Reference Signal}
  \acro{D2DM}{D2D Mode}
  \acro{DMS}{D2D Mode Selection}
  \acro{DPC}{Dirty Paper Coding}
  \acro{DRA}{Dynamic Resource Assignment}
  \acro{DSA}{Dynamic Spectrum Access}
  \acro{FDD}{frequency division duplexing}
  \acro{LTE}{Long Term Evolution}
  \acro{LSAS}{large scale antenna system}
  \acro{LTE}{Long Term Evolution}
  \acro{METIS}{Mobile Enablers for the Twenty-Twenty Information Society}
  \acro{MIMO}{Multiple-input multiple-output}
  \acro{MMSE}{minimum mean squared error}
  \acro{MU-MIMO}{multiuser MIMO}
  \acro{SUMIMO}{single-user multiple-input multiple-output}
  \acro{MISO}{multiple-input single-output}
  \acro{mmWave}{millimeter-wave}
  \acro{MRC}{maximum ratio combining}
  \acro{MS}{mode selection}
  \acro{MSE}{mean square error}
  \acro{MTC}{machine type communications}
  \acro{NSPS}{national security and public safety}
  \acro{NWC}{network coding}
  \acro{PC}{pilot contamination}
  \acro{PHY}{physical layer}
  \acro{QoS}{Quality of Service}
  \acro{QPSK}{Quadri-Phase Shift Keying}
  \acro{RAISES}{Reallocation-based Assignment for Improved Spectral Efficiency and Satisfaction}
  \acro{RAN}{Radio Access Network}
  \acro{RA}{Resource Allocation}
  \acro{RAT}{Radio Access Technology}
  \acro{RB}{resource block}
  \acro{RF}{radio frequency}
  \acro{SINR}{signal-to-noise-and-interference ratio}
  \acro{SNR}{signal-to-noise ratio}
  \acro{STC}{space-time coding}
  \acro{TDD}{time division duplexing}
  \acro{UE}{user equipment}
  \acro{UL}{uplink}
  \acro{VUE}{vehicular user equipment}
  \acro{V2X}{vehicle-to-vehicle and vehicle-to-infrastructure}
  \acro{ZF}{Zero-Forcing}
  \acro{ZMCSCG}{Zero Mean Circularly Symmetric Complex Gaussian}
  \acro{B}{base station}
  \acro{U}{user equipment}
\end{acronym}
%\end{singlespace}



==> reducing-initial-cell (1)/Components/MetaFiles/acronyms.tex <==
%\chapter*{Acronyms}
%\renewcommand{\titulonome}{Acronyms}%
%\renewcommand{\prepbynome}{UFC.33 Team}%

%\begin{singlespace}
\begin{acronym}[LTE-Advanced]%\addtolength{\itemsep}{-0.5\baselineskip}
  \acro{2G}{Second Generation}
  \acro{3G}{3$^\text{rd}$~Generation}
  \acro{3GPP}{3$^\text{rd}$~Generation Partnership Project}
  \acro{4G}{4$^\text{th}$~Generation}
  \acro{5G}{5$^\text{th}$~Generation}
  \acro{AoA}{angle of arrival}
  \acro{AoD}{angle of departure}
  \acro{BER}{bit error rate}
  \acro{BF}{beamforming}
  \acro{BLER}{BLock Error Rate}
  \acro{BPC}{Binary Power Control}
  \acro{BPSK}{Binary Phase-Shift Keying}
  \acro{BRA}{Balanced Random Allocation}
  \acro{BS}{base station}
  \acro{CAP}{Combinatorial Allocation Problem}
  \acro{CAPEX}{Capital Expenditure}
  \acro{CBF}{Coordinated Beamforming}
  \acro{CS}{Coordinated Scheduling}
  \acro{CSI}{channel state information}
  \acro{CSIT}{channel state information at the transmitter}
  \acro{CSIR}{channel state information at the receiver}
  \acro{D2D}{device-to-device}
  \acro{DCA}{Dynamic Channel Allocation}
  \acro{DE}{Differential Evolution}
  \acro{DFT}{Discrete Fourier Transform}
  \acro{ULA}{uniform linear array}
  \acro{DIST}{Distance}
  \acro{DL}{downlink}
  \acro{DMA}{Double Moving Average}
  \acro{DMRS}{Demodulation Reference Signal}
  \acro{D2DM}{D2D Mode}
  \acro{DMS}{D2D Mode Selection}
  \acro{DPC}{Dirty Paper Coding}
  \acro{DRA}{Dynamic Resource Assignment}
  \acro{DSA}{Dynamic Spectrum Access}
  \acro{FDD}{frequency division duplexing}
  \acro{LTE}{Long Term Evolution}
  \acro{LSAS}{large scale antenna system}
  \acro{LTE}{Long Term Evolution}
  \acro{METIS}{Mobile Enablers for the Twenty-Twenty Information Society}
  \acro{MIMO}{Multiple-input multiple-output}
  \acro{MMSE}{minimum mean squared error}
  \acro{MU-MIMO}{multiuser MIMO}
  \acro{SUMIMO}{single-user multiple-input multiple-output}
  \acro{MISO}{multiple-input single-output}
  \acro{mmWave}{millimeter-wave}
  \acro{MRC}{maximum ratio combining}
  \acro{MS}{mode selection}
  \acro{MSE}{mean square error}
  \acro{MTC}{machine type communications}
  \acro{NSPS}{national security and public safety}
  \acro{NWC}{network coding}
  \acro{PC}{pilot contamination}
  \acro{PHY}{physical layer}
  \acro{QoS}{Quality of Service}
  \acro{QPSK}{Quadri-Phase Shift Keying}
  \acro{RAISES}{Reallocation-based Assignment for Improved Spectral Efficiency and Satisfaction}
  \acro{RAN}{Radio Access Network}
  \acro{RA}{Resource Allocation}
  \acro{RAT}{Radio Access Technology}
  \acro{RB}{resource block}
  \acro{RF}{radio frequency}
  \acro{SINR}{signal-to-noise-and-interference ratio}
  \acro{SNR}{signal-to-noise ratio}
  \acro{STC}{space-time coding}
  \acro{TDD}{time division duplexing}
  \acro{UE}{user equipment}
  \acro{UL}{uplink}
  \acro{VUE}{vehicular user equipment}
  \acro{V2X}{vehicle-to-vehicle and vehicle-to-infrastructure}
  \acro{ZF}{Zero-Forcing}
  \acro{ZMCSCG}{Zero Mean Circularly Symmetric Complex Gaussian}
  \acro{B}{base station}
  \acro{U}{user equipment}
\end{acronym}
%\end{singlespace}



==> reducing-initial-cell (1)/Components/MetaFiles/commands.tex <==
% ===========================================================================
% File Name: commands.tex
% File Creation Date: 15.6.1995
% Author: Markku Juntti
% Description: Includes useful commands for Latex edition.
% ===========================================================================


% Theorem-like environments
\IEEEoverridecommandlockouts
\newtheorem{thm}{Theorem}
\newtheorem{prop}{Proposition}
\newtheorem{lem}{Lemma}
\newtheorem{cor}{Corollary}
\newtheorem{defi}{Definition}
\newtheorem{rmk}{Remark}

\def\l{\left}
\def\r{\right}
\def\({\left(}
\def\){\right)}
\def\lb{\left\{}
\def\rb{\right\}}
\def\[{\left[}
\def\]{\right]}

\newcommand{\tred}[1]{\textcolor{red}{#1}}
\newcommand{\tblue}[1]{\textcolor{blue}{#1}}
% Equations, arrays, symbols etc.
\newcommand{\be}{\begin{equation}}
\newcommand{\ee}{\end{equation}}
\newcommand{\ba}{\begin{array}}
\newcommand{\ea}{\end{array}}
\newcommand{\bea}{\begin{eqnarray}}
\newcommand{\eea}{\end{eqnarray}}
\newcommand{\netsize}[3]{#1x#2~#3$^2$}
\newcommand{\combin}[2]{\ensuremath{ \left( \ba{c} #1 \\ #2 \ea \right) }}
   % number of combinations, i.e., polynomial expansion factor
\newcommand{\diag}{{\mbox{diag}}}
\newcommand{\rank}{{\mbox{rank}}}
\newcommand{\dom}{{\mbox{dom{\color{white!100!black}.}}}}
\newcommand{\range}{{\mbox{range{\color{white!100!black}.}}}}
\newcommand{\image}{{\mbox{image{\color{white!100!black}.}}}}
\newcommand{\herm}{^{\mbox{\scriptsize H}}}  % Hermitian transpose
\newcommand{\sherm}{^{\mbox{\tiny H}}}       % Hermitian for subscripts
\newcommand{\tran}{^{\mbox{\scriptsize T}}}  % transpose
\newcommand{\tranIn}{^{\mbox{-\scriptsize T}}}  % transpose
%\newcommand{\gtrless}{>}   % transpose for subscripts
\newcommand{\card}{{\mbox{\textbf{card}}}}
\newcommand{\asign}{{\mbox{$\colon\hspace{-2mm}=\hspace{1mm}$}}}
\newcommand{\ssum}[1]{\mathop{ \textstyle{\sum}}_{#1}}


% Sets of numbers
\newcommand{\vbar}{\raisebox{.17ex}{\rule{.04em}{1.35ex}}}
\newcommand{\vbarind}{\raisebox{.01ex}{\rule{.04em}{1.1ex}}}
%\newcommand{\R}{\ifmmode {\rm I}\hspace{-.2em}{\rm R} \else ${\rm I}\hspace{-.2em}{\rm R}$ \fi}
\newcommand{\D}{\ifmmode {\rm I}\hspace{-.2em}{\rm D} \else ${\rm I}\hspace{-.2em}{\rm D}$ \fi}
\newcommand{\T}{\ifmmode {\rm I}\hspace{-.2em}{\rm T} \else ${\rm I}\hspace{-.2em}{\rm T}$ \fi}
%\newcommand{\N}{\ifmmode {\rm I}\hspace{-.2em}{\rm N} \else \mbox{${\rm I}\hspace{-.2em}{\rm N}$} \fi}
%\newcommand{\B}[1]{\ifmmode {\rm I}\hspace{-.2em}{\rm B}^{#1} \else \mbox{${\rm I}\hspace{-.2em}{\rm B}^{#1}$} \fi}
\newcommand{\B}{\ifmmode {\rm I}\hspace{-.2em}{\rm B} \else \mbox{${\rm I}\hspace{-.2em}{\rm B}$} \fi}
\newcommand{\Hil}{\ifmmode {\rm I}\hspace{-.2em}{\rm H} \else \mbox{${\rm I}\hspace{-.2em}{\rm H}$} \fi}
\newcommand{\Cind}{\ifmmode \hspace{.2em}\vbarind\hspace{-.25em}{\rm C} \else \mbox{$\hspace{.2em}\vbarind\hspace{-.25em}{\rm C}$} \fi}
\newcommand{\Q}{\ifmmode \hspace{.2em}\vbar\hspace{-.31em}{\rm Q} \else \mbox{$\hspace{.2em}\vbar\hspace{-.31em}{\rm Q}$} \fi}
%\newcommand{\Z}{\ifmmode {\rm\bf Z} \else \mbox{{\rm\bf Z}} \fi}
\newcommand{\Z}{\ifmmode {\rm Z}\hspace{-.28em}{\rm Z} \else ${\rm Z}\hspace{-.38em}{\rm Z}$ \fi}

% Functions
\newcommand{\sgn}{\mbox {sgn}}
\newcommand{\var}{\mbox {var}}
\newcommand{\E}{\mbox {E}}
\newcommand{\cov}{\mbox {cov}}
\renewcommand{\Re}{\mbox {Re}}
\renewcommand{\Im}{\mbox {Im}}
\newcommand{\cum}{\mbox {cum}}

% Bold-face Greek letters
\renewcommand{\vec}[1]{{\bf{#1}}}     %equation styles %vector/matrix
\newcommand{\vecsc}[1]{\mbox {\boldmath \scriptsize $#1$}}     %equation styles %vector/matrix
%\newcommand{\vecsc}[1]{\mbox {\bf \scriptsize #1}}
%\newcommand{\itvec}[1]{\mathbf{#1}}     %equation styles %vector/matrix
\newcommand{\itvec}[1]{\mbox {\boldmath $#1$}}
\newcommand{\itvecsc}[1]{\mbox {\boldmath $\scriptstyle #1$}}
\newcommand{\gvec}[1]{\mbox{\boldmath $#1$}}

\newcommand{\balpha}{\mbox {\boldmath $\alpha$}}
\newcommand{\bbeta}{\mbox {\boldmath $\beta$}}
\newcommand{\bgamma}{\mbox {\boldmath $\gamma$}}
\newcommand{\bdelta}{\mbox {\boldmath $\delta$}}
\newcommand{\bepsilon}{\mbox {\boldmath $\epsilon$}}
\newcommand{\bvarepsilon}{\mbox {\boldmath $\varepsilon$}}
\newcommand{\bzeta}{\mbox {\boldmath $\zeta$}}
\newcommand{\boldeta}{\mbox {\boldmath $\eta$}}
\newcommand{\btheta}{\mbox {\boldmath $\theta$}}
\newcommand{\bvartheta}{\mbox {\boldmath $\vartheta$}}
\newcommand{\biota}{\mbox {\boldmath $\iota$}}
\newcommand{\blambda}{\mbox {\boldmath $\lambda$}}
\newcommand{\bmu}{\mbox {\boldmath $\mu$}}
\newcommand{\bnu}{\mbox {\boldmath $\nu$}}
\newcommand{\bxi}{\mbox {\boldmath $\xi$}}
\newcommand{\bpi}{\mbox {\boldmath $\pi$}}
\newcommand{\bvarpi}{\mbox {\boldmath $\varpi$}}
\newcommand{\brho}{\mbox {\boldmath $\rho$}}
\newcommand{\bvarrho}{\mbox {\boldmath $\varrho$}}
\newcommand{\bsigma}{\mbox {\boldmath $\sigma$}}
\newcommand{\bvarsigma}{\mbox {\boldmath $\varsigma$}}
\newcommand{\btau}{\mbox {\boldmath $\tau$}}
\newcommand{\bupsilon}{\mbox {\boldmath $\upsilon$}}
\newcommand{\bphi}{\mbox {\boldmath $\phi$}}
\newcommand{\bvarphi}{\mbox {\boldmath $\varphi$}}
\newcommand{\bchi}{\mbox {\boldmath $\chi$}}
\newcommand{\bpsi}{\mbox {\boldmath $\psi$}}
\newcommand{\bomega}{\mbox {\boldmath $\omega$}}

% Bold italic Roman letters
\newcommand{\bolda}{\mbox {\boldmath $a$}}
\newcommand{\bb}{\mbox {\boldmath $b$}}
\newcommand{\bc}{\mbox {\boldmath $c$}}
\newcommand{\bd}{\mbox {\boldmath $d$}}
\newcommand{\bolde}{\mbox {\boldmath $e$}}
\newcommand{\boldf}{\mbox {\boldmath $f$}}
\newcommand{\bg}{\mbox {\boldmath $g$}}
\newcommand{\bh}{\mbox {\boldmath $h$}}
\newcommand{\bp}{\mbox {\boldmath $p$}}
\newcommand{\bq}{\mbox {\boldmath $q$}}
\newcommand{\br}{\mbox {\boldmath $r$}}
%\newcommand{\bs}{\mbox {\boldmath $s$}}
\newcommand{\bt}{\mbox {\boldmath $t$}}
\newcommand{\bu}{\mbox {\boldmath $u$}}
\newcommand{\bv}{\mbox {\boldmath $v$}}
\newcommand{\bw}{\mbox {\boldmath $w$}}
\newcommand{\bx}{\mbox {\boldmath $x$}}
\newcommand{\by}{\mbox {\boldmath $y$}}
\newcommand{\bz}{\mbox {\boldmath $z$}}

\newenvironment{Ex}
{\begin{adjustwidth}{0.04\linewidth}{0cm}
\begingroup\small
\vspace{-1.0em}
\raisebox{-.2em}{\rule{\linewidth}{0.3pt}}
\begin{example}
}
{
\end{example}
\vspace{-5mm}
\rule{\linewidth}{0.3pt}
\endgroup
\end{adjustwidth}}


\newcommand{\Hossein}[1]{{\textcolor{blue}{\emph{**Hossein: #1**}}}}
\newcommand{\HosseinC}[1]{{\textcolor{blue}{**Hossein: #1**}}}
\newcommand{\Carlo}[1]{{\textcolor{red}{\emph{**Carlo: #1**}}}}
\newcommand{\Yanpeng}[1]{{\textcolor{red}{\emph{**Yanpeng: #1**}}}}
\newcommand{\Challenge}[1]{{\textcolor{red}{#1}}}
\newcommand{\NEW}[1]{{\textcolor{blue}{#1}}}
\newcommand{\new}[1]{{\textcolor{blue}{#1}}}
%\newcommand{\comment}[1]{{\textcolor{red}{**Comment: #1**}}}

%\newenvironment{test}
%{Test begins here: \begingroup \[}
%{\] \endgroup \\ The example has endedd.}

\makeatletter
\let\save@mathaccent\mathaccent
\newcommand*\if@single[3]{%
  \setbox0\hbox{${\mathaccent"0362{#1}}^H$}%
  \setbox2\hbox{${\mathaccent"0362{\kern0pt#1}}^H$}%
  \ifdim\ht0=\ht2 #3\else #2\fi
  }
%The bar will be moved to the right by a half of \macc@kerna, which is computed by amsmath:
\newcommand*\rel@kern[1]{\kern#1\dimexpr\macc@kerna}
%If there's a superscript following the bar, then no negative kern may follow the bar;
%an additional {} makes sure that the superscript is high enough in this case:
\newcommand*\widebar[1]{\@ifnextchar^{{\wide@bar{#1}{0}}}{\wide@bar{#1}{1}}}
%Use a separate algorithm for single symbols:
\newcommand*\wide@bar[2]{\if@single{#1}{\wide@bar@{#1}{#2}{1}}{\wide@bar@{#1}{#2}{2}}}
\newcommand*\wide@bar@[3]{%
  \begingroup
  \def\mathaccent##1##2{%
%Enable nesting of accents:
    \let\mathaccent\save@mathaccent
%If there's more than a single symbol, use the first character instead (see below):
    \if#32 \let\macc@nucleus\first@char \fi
%Determine the italic correction:
    \setbox\z@\hbox{$\macc@style{\macc@nucleus}_{}$}%
    \setbox\tw@\hbox{$\macc@style{\macc@nucleus}{}_{}$}%
    \dimen@\wd\tw@
    \advance\dimen@-\wd\z@
%Now \dimen@ is the italic correction of the symbol.
    \divide\dimen@ 3
    \@tempdima\wd\tw@
    \advance\@tempdima-\scriptspace
%Now \@tempdima is the width of the symbol.
    \divide\@tempdima 10
    \advance\dimen@-\@tempdima
%Now \dimen@ = (italic correction / 3) - (Breite / 10)
    \ifdim\dimen@>\z@ \dimen@0pt\fi
%The bar will be shortened in the case \dimen@<0 !
    \rel@kern{0.6}\kern-\dimen@
    \if#31
      \overline{\rel@kern{-0.6}\kern\dimen@\macc@nucleus\rel@kern{0.4}\kern\dimen@}%
      \advance\dimen@0.4\dimexpr\macc@kerna
%Place the combined final kern (-\dimen@) if it is >0 or if a superscript follows:
      \let\final@kern#2%
      \ifdim\dimen@<\z@ \let\final@kern1\fi
      \if\final@kern1 \kern-\dimen@\fi
    \else
      \overline{\rel@kern{-0.6}\kern\dimen@#1}%
    \fi
  }%
  \macc@depth\@ne
  \let\math@bgroup\@empty \let\math@egroup\macc@set@skewchar
  \mathsurround\z@ \frozen@everymath{\mathgroup\macc@group\relax}%
  \macc@set@skewchar\relax
  \let\mathaccentV\macc@nested@a
%The following initialises \macc@kerna and calls \mathaccent:
  \if#31
    \macc@nested@a\relax111{#1}%
  \else
%If the argument consists of more than one symbol, and if the first token is
%a letter, use that letter for the computations:
    \def\gobble@till@marker##1\endmarker{}%
    \futurelet\first@char\gobble@till@marker#1\endmarker
    \ifcat\noexpand\first@char A\else
      \def\first@char{}%
    \fi
    \macc@nested@a\relax111{\first@char}%
  \fi
  \endgroup
}
\makeatother


\def\bff{{\bf f}}
\def\bX{{\bf X}}
\def\bp{{\bf p}}
\def\bg{{\bf g}}
\def\bK{{\bf K}}
\def\bk{{\bf k}}
\def\bX{{\bf X}}
\def\bnu{{\boldsymbol \nu}}
\def\bxi{{\boldsymbol \xi}}
\def\btheta{{\boldsymbol \theta}}
\def\bphi{{\boldsymbol \phi}}
\def\bq{{\bf q}}
\def\bn{{\bf n}}
\def\bN{{\bf N}}
\def\bz{{\bf z}}
\def\bZ{{\bf Z}}
\def\bD{{\bf D}}
\def\by{{\bf y}}
\def\bY{{\bf Y}}
\def\bV{{\bf V}}
\def\bW{{\bf W}}
\def\bX{{\bf X}}
\def\bu{{\bf u}}
\def\bh{{\bf h}}
\def\bb{{\bf b}}
\def\bH{{\bf H}}
\def\bP{{\bf P}}
\def\bS{{\bf S}}
\def\bQ{{\bf Q}}
\def\bv{{\bf v}}
\def\bc{{\bf c}}
\def\bC{{\bf C}}
\def\bB{{\bf B}}
\def\bG{{\bf G}}
\def\bF{{\bf F}}
\def\bw{{\bf w}}
\def\bR{{\bf R}}
\def\br{{\bf r}}
\def\bI{{\bf I}}
\def\bE{{\bf E}}
\def\bd{{\bf d}}
\def\bv{{\bf v}}
\def\bA{{\bf A}}
\def\bB{{\bf B}}
\def\ba{{\bf a}}
\def\bU{{\bf U}}
\def\bl{{\bf l}}
\def\bs{{\bf s}}
\def\bt{{\bf t}}
\def\bof{{\bf f}}
\def\bi{{\bf i}}
\def\bx{{\bf x}}
\def\bT{{\bf T}}
\def\bO{{\bf O}}
\def\be{{\bf e}}
\def\bDelta{{\bf \Delta}}
\def\bPsi{{\bf \Psi}}
\def\bkappa{{\bf \kappa}}
\def\balpha{{\boldsymbol \alpha}}
\def\bpsi{{\boldsymbol \psi}}
\def\bupsilon{{\boldsymbol \upsilon}}
\def\bPhi{{\bf \Phi}}
\def\bLambda{{\bf \Lambda}}
\def\bSigma{{\bf \Sigma}}
\def\bOmega{{\bf \Omega}}
\def\bGamma{{\bf \Gamma}}
\def\bUpsilon{{\bf \Upsilon}}
\def\blambda{{\boldsymbol \lambda}}
\def\bgamma{{ \boldsymbol\gamma}}
\def\brho{{\boldsymbol \rho}}
\def\bbeta{{\boldsymbol \beta}}
\newcommand{\cbf}[1]{\mathring{\mathbf{#1}}}
\newcommand{\fns}[0]{\fontsize{7.5pt}{10pt}}
\newcommand{\fnss}[0]{\footnotesize}
\def\ct{{\mathrm{c}}}
\def\tt{{\mathrm{t}}}
\def\zp{{\mathrm{zp}}}
\def\calA{{\mathcal{A}}}
\def\calM{{\mathcal{M}}}
\def\calS{{\mathcal{S}}}
\def\calR{{\mathcal{R}}}
\def\bzero{{\mathbf{0}}}
\def\HH{\mathsf{H}}
\def\Nb{N_{\text{BS}}}
\def\Nu{N_{\text{UE}}}
\def\Thetab{\theta_{\text{BS}}}
\def\Thetau{\theta_{\text{UE}}}
\def\Gb{G_{\text{BS}}}
\def\Gu{G_{\text{UE}}}
\def\argmax{\mathrm{arg}\max}
\def\argmin{\mathrm{arg}\min}
\def\b1{{\bf 1}}
\newcommand{\cf}[1]{\mathring{#1}}
\def\Dfz{{\mathrm{diag} ( \bF \bz)}}
\def\tx{{\mathtt{\scriptsize T}}}
\def\rx{{\mathtt{\scriptsize R}}}
\newcommand{\nss}[1]{\textrm{\scriptsize{#1}}}
\newcommand{\tss}[1]{\textrm{\tiny{#1}}}
\newcommand{\bXi}{\mbox {\boldmath $\Xi$}}

\renewcommand{\IEEEQED}{\IEEEQEDopen}

\newcommand{\etal}[1]{{#1}{~\textit{et al.}}}


==> reducing-initial-cell (1)/Components/MetaFiles/packages.tex <==
%\def \treq {\stackrel{\tiny \Delta}{=}}
%\usepackage{hyperref}
%\usepackage[draft]{hyperref}  %to solve bookmark and URL problem
%\usepackage{flushend}  %align the last page-double column format
%\usepackage[space]{grffile}
%\usepackage{subfigure}


\usepackage{times,latexsym,psfrag,eufrak,dsfont}
\usepackage{epstopdf}
\usepackage{bbm}
\usepackage{siunitx}

\usepackage{gensymb}
\usepackage{amsmath,amssymb,amsfonts,amsthm}
\usepackage{epsfig}
\usepackage{cite}
\usepackage{hhline}
\usepackage{multirow}
%\usepackage{framed}
\usepackage{xcolor}
\usepackage{makecell}
%\usepackage{lipsum}
\usepackage{subcaption}
\usepackage{capt-of}
\usepackage[labelformat=simple]{subcaption}
\renewcommand\thesubfigure{(\alph{subfigure})}
\captionsetup[subfigure]{labelsep = space, font = footnotesize}
\captionsetup{font=footnotesize}
%\captionsetup{subrefformat=parens}
\usepackage{enumerate}
\usepackage{enumitem}
\usepackage{color}
\usepackage{graphicx}
\usepackage{algorithmic}
\usepackage[ruled]{algorithm}
\usepackage{booktabs}
\usepackage{bm}
\usepackage[nolist,printonlyused]{acronym} % GF
\usepackage{colortbl}
\usepackage{tabularx}
\usepackage{float}
\newcolumntype{Y}{>{\centering\arraybackslash}X}

%\usepackage{dblfloatfix}
%\usepackage{stfloats}
%\usepackage[section]{placeins}

\usepackage[T1]{fontenc}
\usepackage[utf8]{inputenc}
\usepackage{comment} %GF
\usepackage[author={Hossein}]{pdfcomment}
\newcommand{\PDFcomment}[2]{\pdfmarkupcomment[markup=Highlight,color=yellow,opacity=90]{#1}{#2}}

\usepackage{pgf}
\usepackage{pgfplots}
\usepackage{tikz}
\usepackage{grffile}
\pgfplotsset{compat=newest}
\usetikzlibrary{plotmarks}
\usepgfplotslibrary{patchplots}
\usetikzlibrary{automata,arrows,positioning,calc,matrix,decorations.markings,decorations.pathreplacing,patterns,arrows.meta}
%\usetikzlibrary{automata,arrows,positioning,calc,matrix,decorations.markings,decorations.pathreplacing,patterns}
 \pgfdeclarepatternformonly{south west lines}{\pgfqpoint{-0pt}{-0pt}}{\pgfqpoint{3pt}{3pt}}{\pgfqpoint{3pt}{3pt}}{
        \pgfsetlinewidth{0.4pt}
        \pgfpathmoveto{\pgfqpoint{0pt}{0pt}}
        \pgfpathlineto{\pgfqpoint{3pt}{3pt}}
        \pgfpathmoveto{\pgfqpoint{2.8pt}{-.2pt}}
        \pgfpathlineto{\pgfqpoint{3.2pt}{.2pt}}
        \pgfpathmoveto{\pgfqpoint{-.2pt}{2.8pt}}
        \pgfpathlineto{\pgfqpoint{.2pt}{3.2pt}}
        \pgfusepath{stroke}}
\makeatletter
\newcommand{\vast}{\bBigg@{3}}
\newcommand{\Vast}{\bBigg@{4}}
\makeatother
\renewcommand{\IEEEQED}{\IEEEQEDopen}


\showoutput
\showboxdepth3


%\usepackage{layouts} 
